{\omega}-Petri nets

We introduce {\omega}-Petri nets ({\omega}PN), an extension of plain Petri nets with {\omega}-labeled input and output arcs, that is well-suited to analyse parametric concurrent systems with dynamic thread creation. Most techniques (such as the Karp and Miller tree or the Rackoff technique) that have been proposed in the setting of plain Petri nets do not apply directly to {\omega}PN because {\omega}PN define transition systems that have infinite branching. This motivates a thorough analysis of the computational aspects of {\omega}PN. We show that an {\omega}PN can be turned into an plain Petri net that allows to recover the reachability set of the {\omega}PN, but that does not preserve termination. This yields complexity bounds for the reachability, (place) boundedness and coverability problems on {\omega}PN. We provide a practical algorithm to compute a coverability set of the {\omega}PN and to decide termination by adapting the classical Karp and Miller tree construction. We also adapt the Rackoff technique to {\omega}PN, to obtain the exact complexity of the termination problem. Finally, we consider the extension of {\omega}PN with reset and transfer arcs, and show how this extension impacts the decidability and complexity of the aforementioned problems.

==> complexity.tex <==
\section{Complexity\label{sec:complexity}}
In this section, we use the results from previous sections to
characterize the complexity of the problems we are interested in.

Due to Lemma~[ReachSetEq]\todo{Insert reference to lemma of previous
section here.}, the (place) boundedness and covering problems have the
same complexity for \wPN as for standard Petri nets (\expsp-complete).

It is known that the deadlock-freedom problem can be reduced to
liveness [CEP1993] and that liveness can be reduced to the
reachability problem in standard Petri nets \cite{Hack74}. These
reductions work by introducing gadgets constructed from standard Petri
nets and work for \wPN also. Since the translation to standard Petri
nets in Section~\ref{sec:solv-cover-place} preserves the set of
reachable markings, it implies that the liveness and deadlock-freedom
problems for \wPN can be reduced to the reachability problem for
standard Petri nets. Characterising the exact complexity of the later
problem has been open for quite some time.

As proved in Theorem~\ref{thm:terminationExpsp}, the termination
problem is \expsp{}-complete for \wPN.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "wPetri"
%%% End: 

